Realistic Website Fingerprinting By Augmenting Network Trace

Website Fingerprinting (WF) is considered a major threat to the anonymity of Tor users (and other anonymity systems). While state-of-the-art WF techniques have claimed high attack accuracies, e.g., by leveraging Deep Neural Networks (DNN), several recent works have questioned the practicality of such WF attacks in the real world due to the assumptions made in the design and evaluation of these attacks. In this work, we argue that such impracticality issues are mainly due to the attacker's inability in collecting training data in comprehensive network conditions, e.g., a WF classifier may be trained only on samples collected on specific high-bandwidth network links but deployed on connections with different network conditions. We show that augmenting network traces can enhance the performance of WF classifiers in unobserved network conditions. Specifically, we introduce NetAugment, an augmentation technique tailored to the specifications of Tor traces. We instantiate NetAugment through semi-supervised and self-supervised learning techniques. Our extensive open-world and close-world experiments demonstrate that under practical evaluation settings, our WF attacks provide superior performances compared to the state-of-the-art; this is due to their use of augmented network traces for training, which allows them to learn the features of target traffic in unobserved settings. For instance, with a 5-shot learning in a closed-world scenario, our self-supervised WF attack (named NetCLR) reaches up to 80% accuracy when the traces for evaluation are collected in a setting unobserved by the WF adversary. This is compared to an accuracy of 64.4% achieved by the state-of-the-art Triplet Fingerprinting [35]. We believe that the promising results of our work can encourage the use of network trace augmentation in other types of network traffic analysis.

==> abstract-00.tex <==
Website Fingerprinting (WF) is considered a major threat to the anonymity of Tor users (and other anonymity systems). 
While state-of-the-art WF techniques have claimed high attack accuracies, e.g., by leveraging Deep Neural Networks (DNN), several recent works have questioned the practicality of such WF attacks in the real world due to the assumptions made in the design and evaluation of these attacks. 
% 
% Website Fingerprinting (WF) attacks are a significant threat against the anonymity of Tor users. Deep Neural Networks (DNNs) have enabled WF attacks to achieve extremely high accuracy.
% % with techniques such as Deep Fingerprinting (DF) achieving $98\%$ accuracy in a closed world scenario.  
% However, existing WF techniques lack realistic assumptions making them impractical in real-world scenarios. 
In this work, we identify the root cause of such impracticality issues: the attacker's lack of a longitudinal perspective into network traffic during training of WF classifiers, e.g., a WF classifier may be trained only on high-bandwidth samples but deployed on connections with varying bandwidths in practice. 
% In particular, the traces used during the training phase may be collected in a vastly different setting than those encountered by the attacker during deployment.
We show, for the first time, that such impracticality issues can be alleviated by \emph{augmenting} the network traces used to train WF classifiers. 
Specifically, we introduce \aug, an augmentation technique tailored to the specifications of Tor traces.
We instantiate \aug through semi-supervised and self-supervised learning techniques.
% which we call \netfm and \ourWF, respectively.
% \ali{For Amir: We just mentioned \ourWF in introduction. }
% We then propose \ourWF, a WF attack based on self-supervised learning and augmentation.
Our extensive open-world and close-world experiments demonstrate that under realistic evaluation settings, our WF attacks provide superior performances compared to the state-of-the-art; this is due to their use of augmented network traces for training, which allows them to learn the features of target traffic in unobserved settings (e.g., unknown bandwidth, Tor circuits, etc.).   
For instance, with a 5-shot learning in a closed-world scenario, our self-supervised WF attack (named \ourWF) reaches up to $80\%$  accuracy when the traces for evaluation are collected in a setting unobserved by the WF adversary. This is compared to an accuracy of $64.4\%$ achieved by the state-of-the-art Triplet Fingerprinting~\cite{sirinam2019triplet}.
% Additionally, our results indicate that \ourWF is more robust against \drf comparing to existing systems. 
We believe that the promising results of our work can encourage the use of network trace augmentation in other types of network traffic analysis. 
% The overall results suggest that augmentation is an effective solution for helping a WF attacker to learn unobserved settings that may encounter during deployment. 
% On top of that, we believe that an augmentation tailored to any traffic analysis scenario helps the data collection capability of such systems. 



==> df-aug.tex <==
\subsection{Effect of Augmentation}
In this part, we study the effect of \aug on the conventional WF classification problem. In particular, we want to show how much benefit we get just from \aug without modifying the training procedure (pre-training and fine-tuning of \ourWF) and network architecture. 
To do so, we evaluate the performance of the DF on augmented traces of AWF-{attack} dataset. 
For each value of $N$, we augment the labeled traces such that there are 500 traces per website which is similar to the size of AWF-{pre-training} dataset that is used in \ourWF. This is due to enabling a benchmark for a fair comparison.   

Table~\ref{tab:df-aug} compares the performance of DF trained on augmented traces with DF trained on only labeled traces and \ourWF on \lowbw and \highbw traces. The results show that augmenting the traces using \aug improves the performance of DF without any sophisticated training procedure of \ourWF. This indicates that \aug is beneficial on its own in that it can extend the dataset and make the DF model perform better on unobserved traces. However, using \aug combined with the \ourWF training procedure improves the performance of the WF attack further, particularly on \lowbw traces. 

% \begin{table}
%     \centering
%     \caption{Effect of Augmentation. All numbers are $\%$.}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{@{}l|ll|ll|ll@{}}
%         \toprule
%          & DF~\cite{sirinam2018deep} & & DF \footnotesize{(augmented data}) & & \ourWF \\
%          % \midrule
%          \cmidrule{2-7}
%          % \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
%         % N & \Lowbw(\%) & \Highbw(\%) & \Lowbw(\%) & \Highbw(\%) & \Lowbw(\%) & \Highbw(\%) \\
%         N & \Lowbw & \Highbw & \Lowbw & \Highbw & \Lowbw & \Highbw \\
%          \cmidrule(r){1-1}\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
%         5 & $47.7$ & $55.3$ & $65.5$ & $80.2$ & $\bm{80.2}$ & $\bm{90.9}$  \\
%         10 & $64.6$ & $77.8$ & $72.9$ & $88.3$ & $\bm{85.4}$ & $\bm{94.4}$ \\
%         20 & $73.6$ & $86.9$ & $77.3$ & $92.6$ & $\bm{87.1}$ & $\bm{96.1}$  \\
%         % 90 & $61.9 \pm 0.8$ & $92.6 \pm 0.6 $ & $56.2 \pm 0.5$ & $84.8 \pm 0.4$ & $\bm{79.6 \pm 0.3}$ & $\bm{98.3 \pm 0.1}$ \\
%         \bottomrule
%     \end{tabular}
%     }
%     \label{tab:df-aug}
% \end{table}


==> df-same-data.tex <==
\subsection{Fairer Comparison with DF}
In this part, we provide a fairer comparison between DF and \ourWF by training DF on the same amount of labeled data as the pre-training and fine-tuning dataset of \ourWF.
Although an adversary can fine-tune the pre-trained \ourWF on any dataset and achieves high accuracy as we showed in Section~\ref{sec:cw}, we also consider the AWF-{pre-training} as another source of labeled dataset and train DF on both AWF-{pre-training} and AWF-{attack}. 

Table~\ref{tab:df-same-data} compares the accuracy of DF when trained on both AWF-{pre-training} and AWF-{attack} with \ourWF and DF when trained only on AWF-{attack}. 
To enable a fair comparison with TF and \ourWF we only test DF on AWF-{attack} dataset since AWF-{attack} contains the target websites that the adversary is interested in. 
The results indicate that even when DF is trained on the same amount of data as \ourWF pre-training and fine-tuning data, \ourWF reaches higher accuracy on both \lowbw and \highbw traces for all values of $N$. 
% Note that for smaller values of $N$ DF has even worse performance compared to when it is trained only on AWF-{attack}. 
Note that other than the worse performance of DF in this scenario, the training time for DF is much more than \ourWF. Table~\ref{tab:df-same-data} also compares the training time of both DF and \ourWF and we see that the training of DF is two orders of magnitude slower than \ourWF. This is because the training procedure of \ourWF where the adversary needs to only fine-tune the pre-trained model on the labeled traces whereas DF trains the model from scratch on the whole dataset.
Note that another advantage of \ourWF is that the adversary does not require any labeled traces to perform pre-training as opposed to DF where the adversary needs a huge labeled dataset. 


% \begin{table*}
%     \centering
%     \caption{Comparison with same data. All numbers are $\%$.}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{@{}l|lll|lll|lll@{}}
%         \toprule
%          & DF~\cite{sirinam2018deep} & & & TF~\cite{sirinam2019triplet} & & & \ourWF \\
%          % \midrule
%          \cmidrule{2-10}
%         N & \Lowbw(\%) & \Highbw(\%) & Training Time(s) & \Lowbw(\%) & \Highbw(\%) & Training Time(s) & \Lowbw(\%) & \Highbw(\%) & Training Time(s)\\
%         % N & \Lowbw & \Highbw & Training Time & \Lowbw & \Highbw & Training Time & \Lowbw & \Highbw & Training Time \\
%          \cmidrule(r){1-1}\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
%         5 & $40.4 \pm 1$ &  $55.2 \pm 1.9$ & $465.4$ & $64.4 \pm 0.9$ & $77.9 \pm 0.5$ & -- & $\bm{80.2 \pm 0.6}$ & $\bm{90.9 \pm 0.3}$ & $3.2$ \\
%         10 & $53.5 \pm 1$ & $71.6 \pm 1.1$ & $469.4$ & $69.1 \pm 0.3$ & $83.3 \pm 0.6$ & -- & $\bm{85.4 \pm 0.9}$ & $\bm{94.4 \pm 0.4}$ & $6.5$ \\
%         20 & $63.6 \pm 1.1$ & $81.7 \pm 0.6$ & $475.2$ & $73.9 \pm 0.6$ & $87.8 \pm 0.5$ & -- & $\bm{87.1 \pm 0.4}$ & $\bm{96.1 \pm 0.1}$ & $13.7$\\
%         90 & $77.5 \pm 0.5$ & $92.5 \pm 0.1$ & $518.3$ & $79.2 \pm 0.1$ & $92.5 \pm 0.1$ & -- & $\bm{92.6 \pm 0.4}$ & $\bm{98}$ & $60.6$\\
%         \bottomrule
%     \end{tabular}
%     }
%     \label{tab:df-same-data}
% \end{table*}


% \begin{table}
%     \centering
%     \caption{Effect of Augmentation. All numbers are $\%$.}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{@{}l|ll|ll|ll@{}}
%         \toprule
%          & DF~\cite{sirinam2018deep} & & TF~\cite{sirinam2019triplet} & & \ourWF \\
%          % \midrule
%          \cmidrule{2-7}
%          % \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
%         % N & \Lowbw(\%) & \Highbw(\%) & \Lowbw(\%) & \Highbw(\%) & \Lowbw(\%) & \Highbw(\%) \\
%         N & \Lowbw & \Highbw & \Lowbw & \Highbw & \Lowbw & \Highbw \\
%          \cmidrule(r){1-1}\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
%         5 & $40.4 \pm 1$ & $55.2 \pm 1.9$ & $64.4 \pm 0.9$ & $77.9 \pm 0.5$ & $\bm{80.2 \pm 0.6}$ & $\bm{90.9 \pm 0.3}$  \\
%         10 & $53.5 \pm 1$ & $71.6 \pm 1.1$ & $69.1 \pm 0.3$ & $83.3 \pm 0.6$ & $\bm{85.4 \pm 0.9}$ & $\bm{94.4 \pm 0.4}$ \\
%         20 & $63.6 \pm 1.1$ & $81.7 \pm 0.6$ & $73.9 \pm 0.6$ & $87.8 \pm 0.5$ & $\bm{87.1 \pm 0.4}$ & $\bm{96.1 \pm 0.1}$  \\
%         90 & $77.5 \pm 0.5$ & $92.5 \pm 0.1$ & $79.2 \pm 0.1$ & $92.5 \pm 0.1$ & $\bm{92.6 \pm 0.4}$ & $\bm{98}$ \\
%         \bottomrule
%     \end{tabular}
%     }
%     \label{tab:df-aug}
% \end{table}


==> misc/back_mot.tex <==
\section{Background}\label{back}
% review the problems we have 
% introduce NetCLR
% discuss augmentation
% discuss superior and inferior traces
% \section{Background}\label{back}
Sections \ref{sub:semi} and \ref{sub:self} discuss recent \semi and \self techniques that we use to design our attacks.
% Section \ref{sub:wf} discussed the current literature in WF.

% Section \ref{sub:drift} discusses different types of concept drift that impacts WF attacks.
% Section \ref{sub:threat} describes the threat model for our attacks.

% -------------------------------------------------------------------------
\subsection{Semi-Supervised Learning}\label{sub:semi}

Semi-supervised learning (\semi) is an approach to machine learning that combines a small amount of labeled data with a large amount of unlabeled data during training. \semi mitigates the requirement for labeled data by providing a means of leveraging unlabeled data. 
There is a line of research in \semi aiming at producing an artificial label for unlabeled samples and training the model to predict the artificial label when fed unlabeled images as input~\cite{lee2013pseudo, mclachlan1975iterative, xie2020self, rosenberg2005semi, scudder1965probability}. These approaches are called pseudo-labeling. 
Similarly, consistency regularization~\cite{bachman2014learning, laine2016temporal, sajjadi2016regularization} obtains an artificial label using the model's predicted distribution after randomly modifying the input or model function. 
FixMatch~\cite{sohn2020fixmatch} is a recent \semi algorithm in computer vision that combines consistency regularization and pseudo-labeling and performs a separate \textit{weak} and \textit{strong} augmentation when performing consistency regularization. 
FixMatch produces pseudo labels based on a weakly-augmented unlabeled sample which is used as a target when the model is fed a strongly-augmented version of the same input.
Note that in computer vision, augmentation refers to distorting the pixels of an image to generate new samples with the same label. This includes making small changes to images or using deep learning models to generate new data points. 
In FixMatch, weak augmentation is a standard flip-and-shift augmentation strategy while strong augmentation is based on an algorithm called AutoAugment~\cite{cubuk2019autoaugment}.
% However for network traces, due to their underlying protocol constraints and the nature of the packets augmentation is challenging. We will discuss our augmentation strategy in Section~\ref{sec:aug}.

For an $L$-class classification problem, let $\mathcal{X} = \big\{ (x_b,p_b): b \in (1,\cdots,B) \big\}$ be a batch of $B$ labeled samples, where $x_b$ are the training samples and $p_b$ are one-hot labels. 
Let $\mathcal{U} = \big\{  u_b: b \in (1, \cdots, \mu B) \big\}$ be a batch of $\mu B$ unlabeled samples where $\mu$ is a hyperparameter that denotes the ratio of number of unlabeled samples ($\mathcal{U}$) to labeled samples ($\mathcal{X}$). 
We assume $p_m (y|x)$ is the predicted class distribution produced by the underlying model for input $x$ and $H(p,q)$ denotes the cross-entropy between two probability distributions $p$ and $q$. 
FixMatch performs two types of augmentations: strong and weak, denoted by $\mathcal{A}(.)$ and $\alpha(.)$ respectively. 
The FixMatch loss function consists of two cross-entropy loss terms: a supervised loss $\ell_s$ applied to labeled data and an unsupervised loss $\ell_u$. 
In particular, $\ell_s$ can be the standard cross-entropy loss used in traffic analysis classification scenarios (i.e., Website Fingerprinting) on weakly augmented labeled samples:

\begin{align}
    \ell_s = \frac{1}{B} \sum_{b=1}^{B} \text{H} \big( p_b,p_m(y | \alpha(x_b)) \big)
\end{align}

For each unlabeled sample, FixMatch generates a pseudo label which is then used in a standard cross-entropy loss. Given a weakly-augmented version of an unlabeled sample $q_b = p_m (y | \alpha(u_b))$, we compute the model's predicted class distribution. We then use $\hat{q}_b = \arg\max(q_b)$ as a pseudo-label, except we apply the cross-entropy loss against the model's output for strongly-augmented version of $u_b$:

\begin{align}
    \ell_u = \frac{1}{\mu B} \sum_{b=1}^{\mu B} \mathbb{1}\big(\max(q_b) \geq \tau_f \big) \text{H}\big( \hat{q}_b, p_m (y | \mathcal{A}(u_b)) \big)  
\end{align}

\noindent where $\tau_{f}$ is a scalar hyperparameter indicating the threshold above which we retain a pseudo-label. We minimize the following loss: $\ell_s + \lambda_u \ell_u$ where $\lambda_u$ is a fixed scalar hyperparameter denoting the relative weight of the unlabeled loss. 
% ---------------------------------------------------------------------------
\subsection{Self-Supervised Learning}\label{sub:self}

Self-supervised (Unsupervised) learning (\self) tries to learn useful embeddings from unlabeled data. 
Contrastive Learning is a subset of unsupervised learning that aims to learn embeddings by enforcing similar elements to be equal and dissimilar elements to be different. 
SimCLR~\cite{chen2020simple} is a recent framework in computer vision for contrastive learning of visual representations. In particular, SimCLR learns representations (embeddings) of unlabeled data by maximizing agreement between differently augmented views of the same data example via a contrastive loss in the latent space. 
Note that SimCLR does not use any labeled data to learn the representations of input samples.
% Similar to semi-supervised learning, we will discuss augmentation in network traffic domain in Section~\ref{sec:aug}. 
% We apply SimCLR to traffic analysis algorithms to learn embeddings of network traces where there is no labeled data is available. 
SimCLR framework comprises the following four major components:
\begin{itemize}
    \item A stochastic data augmentation module that transforms any given input sample $x$ resulting in two correlated views of the same sample, denoted $\tilde{x}_i$ and $\tilde{x}_j$, which we consider as a positive pair. 
    \item A neural network base encoder $f(.)$ that extracts embeddings from augmented samples. We use the underlying neural works used in traffic analysis algorithms to obtain $e_i = f(\tilde{x}_i)$ where $e_i \in \mathbb{R}^d$ is the output of the underlying neural network before the last layer (The fully connected layer that generates the output probabilities); $e_i$ also represents the sample embedding extracted by the base model. 
    \item A small neural network \textit{projection head} that maps embeddings to the space where contrastive loss is applied. Projection head is a fully connected network with one hidden layer to obtain $z_i = g(e_i) = W^{(2)}\sigma (W^{(1)}e_i)$ where $\sigma$ is a ReLU non-linearity. 
    \item A \textit{contrastive loss} function to maximize the agreement between augmented versions of an unlabeled sample. Given a set $\{ \tilde{x}_k \}$ including a positive pair of examples $\tilde{x}_i$ and $\tilde{x}_j$, the contrastive prediction task aims to identify $\tilde{x}_j$ in $\{ \tilde{x}_k \}_{k \neq i}$ for a given $\tilde{x}_i$.  
\end{itemize}

SimCLR randomly samples a minibatch of $N$ samples and apply contrastive loss on pairs of augmented samples generated from the minibatch, resulting in 2$N$ network traces. To construct the negative samples, given a positive pair, SimCLR considers the other 2$(N-1)$ augmented samples within a minibatch as negative samples. If we assume $\text{sim}(u, v) = u^T v / \lVert u \rVert \lVert v \rVert$ denotes the dot product between $\ell_2$ normalized of vectors $u$ and $v$ (i.e. cosine similarity), the contrastive loss function for a positive pair of samples $(i, j)$ is defined as:

\begin{align}\label{eq:contrasive-loss}
    \ell_{i,j} = - \log \frac{\exp(\text{sim}(z_i, z_j)/\tau_s)}{\sum_{k=1}^{2N} \mathbb{1}_{[k\neq i]}\exp (\text{sim}(z_i, z_k)/\tau_s)}
\end{align}

\noindent where $\mathbb{1}_{[k\neq i]} \in \{0,1\}$ is an indicator function evaluating to 1 iff $k \neq i$ and $\tau_s$ denotes a temperature parameter. The SimCLR work term this loss \textit{NT-Xent} (the normalized temperature-scaled entropy loss). \ardavan{For Amir: is it okay that our loss formula and the formal problem definition in 2.1 and 2.2 are exactly the same as SimCLR and FixMatch papers?}\amir{yes}

% --------------------------------------------------------------------------

\subsection{Website Fingerprinting: An Overview}
\amir{in this section introduce WF, and introduce main works. You can move stuff from 3.1. Then in section 3, mostly talk about major issues , similar to what we have in intro }

\section{Motivation}

In this section, we briefly overview the literature on WF, and we discuss the issues raised against state-of-the-art work on WF. 

\amir{This section needs some reformatting. We introduce and overview WF in 2.3, here  discuss the WF issues, including concept drift (but not just concept drift). then you can talk about adversary model. Use a similar story to what we have in intro. }

% Section \ref{sub:wf} discussed the current literature in WF.

% Section \ref{sub:drift} discusses different types of concept drift that impacts WF attacks.
% Section \ref{sub:threat} describes the threat model for our attacks.



\subsection{Website Fingerprinting}\label{sub:wf}
Website Fingerprinting (WF) aims at detecting the websites visited over encrypted like VPNs, Tor, and other proxies.
\cite{sirinam2018deep, var-cnn, rimmer2017automated, 184463, panchenko2011website, cai2012touching, wang2013improved, panchenko2016website, hayes2016k, wang2016realistically, jansen2018inside, sirinam2019triplet, wang2020high}.
The attack is performed by a passive adversary who monitors the victim's encrypted network traffic, e.g., a malicious ISP or a surveillance agency.
The adversary compares the victim's observed traffic
flow against a set of prerecorded webpage traces, to identify the webpage being browsed.
% Website fingerprinting differs from flow correlation in that the adversary only observes one end of the connection, e.g., the connection between a client and a Tor relay.
Website fingerprinting has been widely studied in the
context of Tor traffic analysis~\cite{rimmer2017automated, sirinam2018deep, var-cnn, panchenko2011website, cai2012touching, wang2013improved, panchenko2016website, hayes2016k, jansen2018inside, sirinam2019triplet, wang2020high}.


Various machine learning classifiers have been used for WF, e.g.,  using KNN~\cite{184463}, SVM~\cite{panchenko2016website}, and random forest~\cite{hayes2016k}.
However, the state-of-the-art WF algorithms use DNNs to perform website fingerprinting~\cite{sirinam2018deep, rimmer2017automated, var-cnn}.
DNN-based WF attacks demonstrated effective performance in both the closed world setting, where the user is assumed to only browse sites in a monitored set, and the more realistic open world setting, where the user might browse any website, whether monitored or not. For instance, Deep Fingerprinting (DF)~\cite{sirinam2018deep} achieves over $98\%$ accuracy in the closed world and over $0.9$ for both precision and recall in the open world by using convolutional neural networks (CNN).
Similarly, Automated Website Fingerprinting (AWF) is another algorithm based on CNNs that achieves over $96\%$ accuracy in closed world scenario. 
To achieve high accuracies, DF and AWF require large amount of training data, i.e., DF uses 800 traces per each website. Furthermore, both AWF and DF assume the traces for the training and test have same distribution, while traces can be collected in different time periods or from different vantage points. 
% As mentioned earlier, requirement of large training data and different distributions of datasets make mentioned WF attacks unrealistic. 

There are recent studies that perform limited-data website fingerprinting~\cite{sirinam2019triplet, oh2021gandalf, var-cnn}, i.e., Var-CNN is a WF attack which uses known ResNets~\cite{He2015DeepRL}, state-of-the-art CNNs in computer vision, as its base architecture and is effective in limited-data scenarios comparing to previous works. 
% As opposed to DF and AWF which only uses direction of packets (series of +1 and -1 denoting the if packet is upstream or downstream respectively) as features, Var-CNN uses direction as well as packet timings and manual statistical features to perform WF.   
In limited-data scenario, Var-CNN can achieve $97.8\%$ accuracy with 100 traces for each website in a closed world scenario. 
Sirinam et al. propose Triplet Fingerprinting (TF)~\cite{sirinam2019triplet} where they examine how an attacker can leverage N-shot learning\textemdash a machine learning technique requiring just a few training samples to identify a given class\textemdash to reduce the amount of data requiring for training as well as mitigate the adverse effects of dealing with different distribution of traces. 
TF leverages triplet networks~\cite{schroff2015facenet}, an image classification method in contrastive learning, to train a feature extractor that maps network traces to fixed length embeddings. TF uses 25 samples per website and 775 websites to train the feature extractor. 
The embeddings are then used to $N$-train a K-Nearest Neighbour (KNN) classifier. 
TF achieves over $92\%$ accuracy using 25 samples per each website to train the feature extractor and only 5 samples to train the KNN classifier.  
% TF also investigates the scenario where the training and test data are from different distributions.
Generative Adversarial Network for Data-Limited Fingerprinting (GANDaLF)~\cite{oh2021gandalf} is a another WF attack proposed by Oh et al. that is effective when few training samples are available. In particular, \gandalf uses a Generative Adversarial Network (GAN) to generate a large set of "fake" network traces which helps to train a DNN in distinguishing between classes of actual training data. In a normal closed world WF setting, \gandalf achieves $87\%$ accuracy using only 20 instances per website (100 sites). 
Online WF~\cite{cherubin2022online} is the most recent WF attack proposed by Cherubin et al. Online WF argues that existing WF techniques lack realistic assumptions making them impractical in real-world scenarios. 
They show that the synthetic traces collected by researchers using automated browsers over entry relays cannot represent the correct distribution of genuine Tor traces.
To address this problem, Online WF uses genuine Tor traces collected over an exit relay to perform a more realistic WF attack.  

In this work, we aim at addressing the root cause of impracticality of existing WF techniques which is the limitation in the adversary's data collection capability. 
As a potential solution, we use data augmentation to enable the model learn even in unobserved settings. We then deploy augmentation through \semi and \self techniques to propose a realistic WF attack. 
% In this work, we address the same issue using contrastive learning and a sophisticated augmentation algorithm which is tailored to the specific characteristics of Tor traces. 

% --------------------------------------------------------------------------
\subsection{Concept Drift}\label{sub:drift}
In a dynamic environment, the distribution of the target variable that a machine learning model learns can be non-stationary and therefore change over time, impacting the performance of the model when deployed. In the literature, this change in the distribution is referred to as dataset shift~\cite{morenotorres2012drift} or concept drift~\cite{gama2014conceptsurvey}.
% Using the terminology of Moreno-Torres et al.~\cite{morenotorres2012drift}
In the classification context, a problem can be defined by a set of covariates $X$, denoting the features, a class (target) variable $y$, and a joint distribution $P(y,X)$ referred to as concept, which can be written as $P(X|y)P(y)$. Therefore, concept drift between time $t_0$ and time $t_1$ can be defined as $\exists X: P_{t_0}(X,y) \neq P_{t_1}(X,y)$, where $P_{t_i}(X,y)$ denotes the joint distribution between X and y at time $t_i$ for $i \in \{0,1\}$. \textit{Real concept drift} is the changes in $P(X|y)$ between $t_0$ and $t_1$ which can happen whether $P(y)$ changes or not. \textit{Virtual concept drift}, also referred to as \textit{covariate shift} and \textit{feature change} happens if $P(X)$ changes between $t_0$ and $t_1$ but $P(y|X)$ does not change.


The data we use for our experiments consists AWF, a large dataset collected in 2017~\cite{rimmer2017automated}, as well a smaller Drift dataset that we collect 5 years later.
Over time, the content of a website change and can be completely different after 5 years, e.g. its back-end can be different resulting in a different loading time. Yet, it still has the same class label (URL), meaning $P(X|y)$ changes over time. Therefore, a deployed WF model needs to be resilient to real concept drift.
Note that this requirement exists whether or not the WF model uses offline learning or online learning. Traditional WF attacks ~\cite{oh2021gandalf, sirinam2019triplet, var-cnn, rimmer2017automated} use offline learning where all of the training data is available at the time of model training. Cherubin et al. ~\cite{cherubin2022online} propose using online learning, where the deployed model is continuously updated as more training data arrives. In either case, in a non-stationary and dynamic environment, the data evolves over time as the content of websites change and new websites are added to the monitored set. Therefore, $P(X|y)$ is changing over time.

Furthermore, our method of collecting traffic and extracting Tor cells for generating traces of a website slightly differs from that of \cite{rimmer2017automated}. For instance, the amount of time we wait for each website to load is different. Consequently, the distribution of traces collected for the same website can vary between the two datasets, even if everything else is the same. In this case, $P(X)$ has changed, but $P(y|X)$ has not changed. This is an instance of virtual concept drift to which our WF model should be resilient.

% --------------------------------------------------------------------------
% \subsection{Threat Model}\label{sub:threat}
% In this work, we consider a passive and local adversary for Tor, similar to Figure \ref{fig:wf}. Network administrators, Internet Service Providers (ISP), and Autonomous Systems (AS) are examples of a local adversary having access to the link between the client and the entry relay. The adversary collects TCP packets from which it can extract Tor cells. We assume that the adversary cannot break the encryption provided by Tor. To evaluate our attack against previous work and defenses, we consider the \textit{closed world} scenario in which the client is assumed to only be visiting one the \textit{monitored} websites that the adversary has trained its model on. For the \textit{open world} evaluation, the client can visit \textit{unmonitored} pages on which the adversary's model has not been trained. We also assume that the client is visiting one web page at a time through Tor. 
% For a WF attack to be practical, the adversary needs flexibility in choosing a new set of monitored websites without having to collect large amounts of data to train a new model. \ourWF which is based on the the self-supervised framework discussed in Section \ref{sub:self}, has a pre-training phase in which the model learns representations of unlabeled Tor traces and a fine-tuning phase to adjust the model to the monitored websites with a limited number of labeled samples. To pre-train \ourWF, the adversary can either use a large publicly available dataset like AWF, or collect its own traffic. This phase of the attack requires more time and resources than the fine-tuning, yet only needs to be done only once and does not need labeled traffic.
% % Then, for a list of monitored websites, the adversary only needs a limited number of labeled traces to fine-tune its pre-trained model.
% For \ourWF to achieve a high performance, the self-supervised model needs to be able to learn high quality representations of Tor traces. This can be challenging due to the changing network conditions and non-stationary distribution of noise in Tor, making the data augmentation crucial for learning good representations.
% Section \ref{sec:aug} describes \aug, our augmentation algorithm which is tailored to the domain of Tor website traffic traces which replicates different network conditions through applying various transformation on Tor traces. 
% To evaluate whether our self-supervised model is learning high quality representations, we partition the traces in our data into a set of \highbw and a set of \lowbw traces based on a metric we describe in Section \ref{sub:network-condition}. We then pre-train the model on only one set of traces. The evaluation results in Section \ref{exp} show that the model performs well on traces collected in network conditions it has not seen in the pre-training phase. This indicates the model was able to learn high quality representations, addressing the limited diversity in network conditions of the training data.
% To evaluate the resilience of \ourWF against concept drift, we pre-train the model on AWF, and fine-tune it on our Drift dataset which we collected 5 years later.



% \subsection{Threat Model}\label{sub:threat}
\subsection{Adversary Model}\label{sub:threat}
In this work, we consider a passive and local adversary for Tor, similar to Figure \ref{fig:wf}. Network administrators, Internet Service Providers (ISP), and Autonomous Systems (AS) are examples of a local adversary having access to the link between the client and the entry relay. The adversary collects TCP packets from which it can extract Tor cells. We assume that the adversary cannot break the encryption provided by Tor.
In machine learning-based WF attacks, the adversary first trains a classification model (mostly DNNs in recent works) and then deploys the model against users' traffic. Figure~\ref{fig:wf} shows the setting of a machine learning-based WF attack. 
As mentioned in Section~\ref{sec:intro}, existing WF attacks do not consider the difference between the setting where evaluation and training traces are collected. This limitation in data collection make the existing threat model impractical in real-world scenarios. 

In this work, the attacker has the same interception point as previous WF attacks. The attacker collect traces by running an entry relay and then use these traces to train a WF classifier. 
\red{Maybe here we can say the problem of Online WF}
However, to evaluate the ability of the attacker to generalize for unobserved settings during deployment, we use traces collected in different network conditions for training and deployment. 
We assume that the attacker use traces that are collected in consistent network conditions with high bandwidth and low latency. Hence, the attacker performs all the training phases on \highbw traces. 
On the other hand, during deployment, the attacker may encounter traces in various network conditions such as low bandwidth and high latency. So to consider the worst case scenario, we evaluate the performance of our attack on \lowbw traces. 
In Section~\ref{sec:data}, we elaborate on how we divide the traces of our dataset into \lowbw and \highbw traces. 
We believe that in such scenario, we evaluate the capability of the model of learning the underlying features of traces in unobserved settings. In Sections~\ref{sec:aug} and \ref{sec:model} we explain how we achieve this goal by leveraging data augmentation and deploy it through \self and \semi algorithms. 


\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{images/WF-training-test.pdf}
  \caption{Setup of a machine learning-based WF attack.}
  \label{fig:wf}
\end{figure}




==> misc/background-00.tex <==
\section{Background}\label{back}

\subsection{Semi-Supervised Learning}

Semi-supervised learning (SSL) is an approach to machine learning that combines a small amount of labeled data with a large amount of unlabeled data during training. SSL mitigates the requirement for labeled data by providing a means of leveraging unlabeled data. 
There is a line of research in semi-supervised learning aiming at producing an artificial label for unlabeled samples and training the model to predict the artificial label when fed unlabeled images as input~\cite{lee2013pseudo, mclachlan1975iterative, xie2020self, rosenberg2005semi, scudder1965probability}. These approaches are called pseudo-labeling. 
Similarly, consistency regularization~\cite{bachman2014learning, laine2016temporal, sajjadi2016regularization} obtains an artificial label using the model's predicted distribution after randomly modifying the input or model function. 
FixMatch~\cite{sohn2020fixmatch} is a recent semi-supervised algorithm in computer vision that combines consistency regularization and pseudo-labeling and performs a separate \textit{weak} and \textit{strong} augmentation when performing consistency regularization. 
FixMatch produces pseudo labels based on a weakly-augmented unlabeled sample which is used as a target when the model is fed a strongly-augmented version of the same input.
Note that in computer vision, augmentation refers to distorting the pixels of an image to generate new samples with the same label. This includes making small changes to images or using deep learning models to generate new data points. 
In FixMatch, weak augmentation is a standard flip-and-shift augmentation strategy while strong augmentation is based on an algorithm called AutoAugment~\cite{cubuk2019autoaugment}.
However for network traces, due to their underlying protocol constraints and the nature of the packets augmentation is challenging. We will discuss our augmentation strategy in Section~\ref{sec:aug}.

For an $L$-class classification problem, let $\mathcal{X} = \big\{ (x_b,p_b): b \in (1,\cdots,B) \big\}$ be a batch of $B$ labeled samples, where $x_b$ are the training samples and $p_b$ are one-hot labels. 
Let $\mathcal{U} = \big\{  u_b: b \in (1, \cdots, \mu B) \big\}$ be a batch of $\mu B$ unlabeled samples where $\mu$ is a hyperparameter that denotes the ratio of number of unlabeled samples ($\mathcal{U}$) to labeled samples ($\mathcal{X}$). 
We assume $p_m (y|x)$ is the predicted class distribution produced by the underlying model for input $x$ and $H(p,q)$ denotes the cross-entropy between two probability distributions $p$ and $q$. 
FixMatch performs two types of augmentations: strong and weak, denoted by $\mathcal{A}(.)$ and $\alpha(.)$ respectively. 
The FixMatch loss function consists of two cross-entropy loss terms: a supervised loss $\ell_s$ applied to labeled data and an unsupervised loss $\ell_u$. 
In particular, $\ell_s$ can be the standard cross-entropy loss used in traffic analysis classification scenarios (i.e., Website Fingerprinting) on weakly augmented labeled samples:

\begin{align}
    \ell_s = \frac{1}{B} \sum_{b=1}^{B} \text{H} \big( p_b,p_m(y | \alpha(x_b)) \big)
\end{align}

As mentioned earlier, for each unlabeled sample, FixMatch generates a pseudo label which is then used in a standard cross-entropy loss. Given a weakly-augmented version of an unlabeled sample $q_b = p_m (y | \alpha(u_b))$, we compute the model's predicted class distribution. We then use $\hat{q}_b = \arg\max(q_b)$ as a pseudo-label, except we apply the cross-entropy loss against the model's output for strongly-augmented version of $u_b$:

\begin{align}
    \ell_u = \frac{1}{\mu B} \sum_{b=1}^{\mu B} \mathbb{1}\big(\max(q_b) \geq \tau_f \big) \text{H}\big( \hat{q}_b, p_m (y | \mathcal{A}(u_b)) \big)  
\end{align}

\noindent where $\tau_{f}$ is a scalar hyperparameter indicating the threshold above which we retain a pseudo-label. We minimize the following loss: $\ell_s + \lambda_u \ell_u$ where $\lambda_u$ is a fixed scalar hyperparameter denoting the relative weight of the unlabeled loss. 

% ---------------------------------------------------------------------------
\subsection{Self-Supervised Learning}

Self-supervised (Unsupervised) representation learning tries to learn useful embeddings from unlabeled data. 
Contrastive Learning is a subset of unsupervised learning that aims to learn embeddings by enforcing similar elements to be equal and dissimilar elements to be different. 
SimCLR~\cite{chen2020simple} is a recent framework in computer vision for contrastive learning of visual representations. In particular, SimCLR learns representations (embeddings) of unlabeled data by maximizing agreement between differently augmented views of the same data example via a contrastive loss in the latent space. 
Note that SimCLR does not use any labeled data to learn the representations of input samples.
% Similar to semi-supervised learning, we will discuss augmentation in network traffic domain in Section~\ref{sec:aug}. 
% We apply SimCLR to traffic analysis algorithms to learn embeddings of network traces where there is no labeled data is available. 
SimCLR framework comprises the following four major components:
\begin{itemize}
    \item A stochastic data augmentation module that transforms any given input sample $x$ resulting in two correlated views of the same sample, denoted $\tilde{x}_i$ and $\tilde{x}_j$, which we consider as a positive pair. 
    \item A neural network base encoder $f(.)$ that extracts embeddings from augmented samples. We use the underlying neural works used in traffic analysis algorithms to obtain $e_i = f(\tilde{x}_i)$ where $e_i \in \mathbb{R}^d$ is the output of the underlying neural network before the last layer (The fully connected layer that generates the output probabilities); $e_i$ also represents the sample embedding extracted by the base model. 
    \item A small neural network \textit{projection head} that maps embeddings to the space where contrastive loss is applied. Projection head is a fully connected network with one hidden layer to obtain $z_i = g(e_i) = W^{(2)}\sigma (W^{(1)}e_i)$ where $\sigma$ is a ReLU non-linearity. 
    \item A \textit{contrastive loss} function to maximize the agreement between augmented versions of an unlabeled sample. Given a set $\{ \tilde{x}_k \}$ including a positive pair of examples $\tilde{x}_i$ and $\tilde{x}_j$, the contrastive prediction task aims to identify $\tilde{x}_j$ in $\{ \tilde{x}_k \}_{k \neq i}$ for a given $\tilde{x}_i$.  
\end{itemize}

SimCLR randomly samples a minibatch of $N$ samples and apply contrastive loss on pairs of augmented samples generated from the minibatch, resulting in 2$N$ network traces. To construct the negative samples, given a positive pair, SimCLR considers the other 2$(N-1)$ augmented samples within a minibatch as negative samples. If we assume $\text{sim}(u, v) = u^T v / \lVert u \rVert \lVert v \rVert$ denotes the dot product between $\ell_2$ normalized of vectors $u$ and $v$ (i.e. cosine similarity), the contrastive loss function for a positive pair of samples $(i, j)$ is defined as:

\begin{align}\label{eq:contrasive-loss}
    \ell_{i,j} = - \log \frac{\exp(\text{sim}(z_i, z_j)/\tau_s)}{\sum_{k=1}^{2N} \mathbb{1}_{[k\neq i]}\exp (\text{sim}(z_i, z_k)/\tau_s)}
\end{align}

\noindent where $\mathbb{1}_{[k\neq i]} \in \{0,1\}$ is an indicator function evaluating to 1 iff $k \neq i$ and $\tau_s$ denotes a temperature parameter. The SimCLR work term this loss \textit{NT-Xent} (the normalized temperature-scaled entropy loss). \ardavan{For Amir: is it okay that our loss formula and the formal problem definition in 2.1 and 2.2 are exactly the same as SimCLR and FixMatch papers?}




% --------------------------------------------------------------------------
\subsection{Website Fingerprinting}
Website Fingerprinting (WF) aims at detecting the websites visited over encrypted like VPNs, Tor, and other proxies.
\cite{sirinam2018deep, var-cnn, rimmer2017automated, 184463, panchenko2011website, cai2012touching, wang2013improved, panchenko2016website, hayes2016k, wang2016realistically, jansen2018inside, sirinam2019triplet, wang2020high}.
The attack is performed by a passive adversary who monitors the victim's encrypted network traffic, e.g., a malicious ISP or a surveillance agency.
The adversary compares the victim's observed traffic
flow against a set of prerecorded webpage traces, to identify the webpage being browsed.
 Website fingerprinting differs from flow correlation in that
the adversary only observes one end of the connection, e.g., the connection between a client and a Tor relay.
Website fingerprinting has been widely studied in the
context of Tor traffic analysis~\cite{rimmer2017automated, sirinam2018deep, var-cnn, panchenko2011website, cai2012touching, wang2013improved, panchenko2016website, hayes2016k, jansen2018inside, sirinam2019triplet, wang2020high}.


Various machine learning classifiers have been used for WF, e.g.,  using KNN~\cite{184463}, SVM~\cite{panchenko2016website}, and random forest~\cite{hayes2016k}.
However, the state-of-the-art WF algorithms use Deep Neural Networks to perform website fingerprinting~\cite{sirinam2018deep, rimmer2017automated, var-cnn}.
DNN-based WF attacks demonstrated effective performance in both the closed-world setting, where the user is assumed to only browse sites in a monitored set, and the more realistic open-world setting, where the user might browse any website, whether monitored or not. For instance, Deep Fingerprinting (DF)~\cite{sirinam2018deep} achieves over $98\%$ accuracy in the closed-world and over $0.9$ for both precision and recall in the open-world by using convolutional neural networks (CNN).
Similarly, Automated Website Fingerprinting (AWF) is another algorithm based on CNNs that achieves over $96\%$ accuracy in closed-world scenario. 
To achieve high accuracies, DF and AWF require large amount of training data, i.e., DF uses 800 traces per each website and 300 traces per website. Furthermore, both AWF and DF assume the traces for the training and test have same distribution, while traces can be collected in different time periods or from different vantage points. As mentioned earlier, requirement of large training data and different distributions of datasets make mentioned WF attacks unrealistic. 

There are recent studies that perform limited-data website fingerprinting~\cite{sirinam2019triplet, oh2021gandalf, var-cnn}, i.e., Var-CNN is a WF attack which uses known ResNets~\cite{He2015DeepRL}, state-of-the-art CNNs in computer vision, as its base DNN architecture which is effective in limited-data scenarios comparing to previous works. 
As opposed to DF and AWF which only uses direction of packets (series of +1 and -1 denoting the if packet is upstream or downstream respectively) as features, Var-CNN uses direction as well as packet timings and manual statistical features to perform WF.   
In limited-data scenario, Var-CNN can achieve $97.8\%$ accuracy with 100 traces for each website in a closed-world scenario. 
Sirinam et al. propose Triplet Fingerprinting (TF)~\cite{sirinam2019triplet} where they examine how an attacker can leverage N-shot learning\textemdash a machine learning technique requiring just a few training samples to identify a given class\textemdash to reduce the amount of data requiring for training as well as mitigate the adverse effects of dealing with different distribution of traces. 
TF leverages triplet networks~\cite{schroff2015facenet}, an image classification method in contrastive learning, to train a feature extractor that maps network traces to fixed length embeddings. TF uses 25 samples per website and 775 websites to train the feature extractor. 
The embeddings are then used to $N$-train a K-Nearest Neighbour (KNN) classifier. 
TF achieves over $92\%$ accuracy using 25 samples per each website to train the feature extractor and only 5 samples to train the KNN classifier.  
% TF also investigates the scenario where the training and test data are from different distributions.
Generative Adversarial Network for Data-Limited Fingerprinting (GANDaLF)~\cite{oh2021gandalf} is a another WF attack proposed by Oh et al. that is effective when few training samples are available. In particular, \gandalf uses a Generative Adversarial Network (GAN) to generate a large set of "fake" network traces which helps to train a DNN in distinguishing between classes of actual training data. In a normal closed-world WF setting, \gandalf achieves $87\%$ accuracy using only 20 instances per website (100 sites). 
Online WF~\cite{cherubin2022online} is the most recent WF attack proposed by Cherubin et al. Online WF uses the same feature extractor as TF and genuine Tor traces collected over and exit relay to perform a more realistic WF attack. They mentioned that the synthetic traces collected by researchers using automated browsers over entry relays cannot represent the correct distribution of genuine Tor traces. 
In this work, we address the same issue using contrastive learning and a sophisticated augmentation algorithm which is tailored to the specific characteristics of Tor traces. 

%-----------------------------------------------------------------------


==> misc/intro-00.tex <==
\section{Introduction}\label{intro}


Anonymous communication systems  hide the identities of the Internet end-points (e.g., websites) visited by Internet users, therefore protecting them  against online tracking, surveillance, and censorship.
Tor~\cite{dingledine2004tor} is  the most popular anonymous communication system in the wild with several million daily  users~\cite{tor-metric}. 
% Tor provides anonymity by relaying clients' traffic through cascades of relays, known as circuits. 
The biggest threat to the anonymity provided by Tor and similar anonymity systems is a class of attacks known as Website Fingerprinting (WF)~\cite{sirinam2018deep, sirinam2019triplet, cherubin2017website, cherubin2022online, oh2021gandalf, rimmer2017automated, panchenko2011website, cai2012touching, wang2013improved, panchenko2016website, hayes2016k, wang2016realistically, oh2019p1, var-cnn, 184463}: 
the adversary (e.g., a surveillance organization) trains a machine learning classifier on network traffic to target Internet websites and uses such a classifier on the anonymized (e.g., Tor) traffic  of Internet users to infer the websites they are visiting. 
State-of-the-art WF attacks claim to achieve high accuracies by leveraging advanced Deep Neural Network (DNN) architectures~\cite{oh2019p1, var-cnn, sirinam2018deep, sirinam2019triplet, cherubin2022online, rimmer2017automated, oh2021gandalf}, e.g., Deep Fingerprinting~\cite{sirinam2018deep} claims a $98\%$ inference accuracy in a closedd world scenario.  

% Website Fingerprinting (WF) attacks are among the most damaging attacks an adversary can perform against Tor to deanonymize the clients and infer their web activity. WF is performed by a passive adversary who monitors the victim's network traffic, e.g., a malicious ISP or surveillance agency. 
% The adversary
% compares the victim's observed traffic trace against a set of prerecorded website traces, to identify the webpage being browsed.



\paragraphb{Critics of WF Studies:}
\red{here you should be more assertive. cite claims from recent works that criticize. say that recent work has criticized the literature on WF due to missing to account for practical assumptions. And then talk about this assertively. Give numbers from those papers on what could happen bc of these miss assumptions}
Despite the promising performance of DNN-based WF attacks, they often lack realistic and practical assumptions in traffic generation, such as taking into account variations in client's browsing behavior, different browser configurations, and variations in world size, while requiring large amounts of labeled data. These factors can significantly degrade the performance of existing WF attacks in real-world scenarios~\cite{juarez2014critical, critique, rimmer2017automated, cherubin2022online}.
To overcome these challenges, researchers have considered more realistic scenarios by using a diverse set of browsers, data freshness techniques~\cite{wang2016realistically}, and other innovative solutions~\cite{wang2016realistically}. 
However, the outstanding performance of these WF attacks still depends on unrealistic scenarios not taking into account issues such as concept drift and dynamic network conditions which can significantly affect the performance of WF attacks.  

Concept drift refers to the phenomenon where the properties that distinguish one website from another can change over time. This can make it more difficult for WF techniques to accurately identify and track individual websites, as the features that were previously used to distinguish them may no longer be reliable. To address concept drift, researchers may need to regularly re-train and update the WF model making the attack infeasible.
Variable network conditions can also impact the performance of WF techniques.
Researchers typically collect ground-truth data for training WF classifiers by generating synthetic network traces through automated browsing of a pre-defined set of websites.
This traffic collection often occurs in networks with stable conditions and high bandwidths, leading to the training of WF classifiers on these \textit{\highbw} traces. However, during deployment, WF classifiers may encounter genuine network traces generated by actual Tor users, which may occur under unstable and poor network conditions and reduce the effectiveness of WF attacks. 
For instance, if a website loads more slowly due to poor network conditions, it may change the timing of certain elements of the page, which could be used as a fingerprinting feature. 
Network conditions also affect the overall appearance of a website, as certain features or elements may not load correctly under certain conditions. 
All of these factors make existing WF attacks more challenging in realistic scenarios where the model is deployed over \textit{\lowbw} traces.

Researchers have used different techniques to overcome these challenges, e.g., Online WF~\cite{cherubin2022online} argue that collecting website traces from Tor entry relays is not realistic and instead, they trained their WF classifier using genuine Tor traces collected from exit relays. However, accessing an exit relay is not always feasible for the attacker due to Tor regulations. 
Furthermore, Sirinam et al.~\cite{sirinam2019triplet} proposed Triplet Fingerprinting (TF) which uses triplet networks to learn representations of website traces. However, TF still lacks realistic assumptions about the website traces that can have variable network conditions for different users in different locations. Moreover, TF requires a large amount of labeled data for its feature extraction. 

\red{To start this part, you have to say that the root cause of the issues mentioned above (e.g drifting) is the lack of access to data in different settings/points; therefore we argue for augmentation (since it's not practical to collect data in all settings)}
\paragraphb{Enabling WF under realistic settings:}
In this work, first, we create a new direction for evaluating WF classifiers in a realistic and practical scenario. We argue that in a realistic scenario, the attacker often trains the WF classifier using traces collected in consistent network conditions (\highbw traces). On the other hand in the deployment phase, the model may encounter traces with various network conditions. Furthermore, the deployment may happen with a huge gap from the time that training samples are collected. Therefore, in a realistic WF scenario, we want a model that is trained on \highbw traces, and capable of performing properly on \lowbw traces.
To achieve this goal, the model needs to generalize its classification ability to traces with unseen distributions in the deployment phase of the attack.
Semi-supervised and self-supervised learning algorithms~\cite{sohn2020fixmatch, chen2020simple} are known to have this ability and, in this work, we utilize them to propose WF attacks that are effective in practical scenarios. 
The core part of these algorithms is data augmentation making them capable of learning useful representations of website traces without the need for large labeled samples.

In our proposed realistic WF scenario, the augmentation needs to reflect different modifications that may happen to traces during the deployment phase due to various realistic conditions mentioned earlier such as concept drift and network conditions. 
Hence it is necessary to use an augmentation that is tailored to specific configurations of the Tor network. We propose \aug, an augmentation algorithm that is specific to the domain of Tor traces. Each rule of \aug represents a realistic scenario that may occur to Tor traces such as content change due to concept drift, packet loss, and packet retransmission in circuits with high latency.
We compare \aug with a random augmentation and show the effect of a tailored augmentation on the performance of the WF classifier. 

\red{here, you say that augmented network traffic can be used in different ways to train WF. We used them in these ways ...}
\paragraphb{Making use of network augmentation:}
We implement several deployments of semi-supervised and self-supervised learning techniques to design a WF attack. After evaluating these systems, we find SimCLR~\cite{chen2020simple} which is based on self-supervised contrastive learning to have the best performance. Therefore, we propose \ourWF, a self-supervised contrastive learning WF algorithm that is integrated with \aug. \ourWF learns useful representationس of Tor traces without any requirement of labeled data as a pre-training phase. We then fine-tune the pre-trained base network in the proposed realistic WF scenario. All the training phases of \ourWF are performed on \highbw traces and our results show that when evaluated on \lowbw traces, \ourWF outperforms existing WF techniques significantly. 
We perform extensive experiments to evaluate \ourWF in both closed world and open world WF scenarios. 
Our results suggest that \ourWF is able to identify visited websites with high accuracy even when the distribution of training and test datasets are different (with 6 years gap), e.g., in a closed world scenario and with only 5 labeled samples, \ourWF has $80\%$ accuracy on \lowbw traces while Triplet Fingerprinting (TF), the state-of-the-art low-data WF technique, reaches only $64.4\%$ in exact same setting.  
\ourWF is also effective in an open world scenario, e.g., when using 5 labeled samples, \ourWF reaches $92\%$ precision while Deep Fingerprinting has only $75\%$ precision.


% ------------------------------------------------------------------
\begin{comment}
In this work, we introduce \ourWF, a WF attack based on contrastive learning and augmentation of network traces. 
\ourWF consists of a pre-training, fine-tuning, and an deployment phase. During pre-training phase, \ourWF learns to generate fixed-size embedding of network traces using various augmented version of unlabeled traces, without the need for labeled samples. This is in contrast to previous approaches, which require labeled samples for their pre-training.
To augment the traces, we propose \aug, an algorithm tailored to the domain of network traces. \aug includes 4 rules of augmentation and each one of them reflect realistic scenarios that may occur to traces during browsing, e.g., website content change due to concept drift or packet retransmission due to high latency. 
Using an augmentation tailored to the specific configurations of the Tor network helps the pre-trained model to encounter distribution of traces that are not present in synthetic traces.
\aug eases the challenges caused by concept drift and variable network conditions by simulating the effects of these concepts on traces through carefully designed augmentation rules. 
Fine-tuning phase is similar to most of the WF attacks. We fine-tune the pre-trained base model using different number of labeled samples.
\end{comment}
% ------------------------------------------------------------------

\begin{comment}
To evaluate \ourWF in realistic scenarios, we perform the whole pre-training and fine-tuning phases on \highbw traces and evaluate it on both \lowbw and \highbw ones. Evaluating on \lowbw traces assess the model's capability to generalize WF to unseen distribution of traces in the deployment phase. 
We perform extensive set of experiments to evaluate \ourWF in both closed world and open world WF scenarios. 
Our results suggest that \ourWF is able to identify visited websites with high accuracy even when the distribution of training and test datasets are different (with 6 years gap), e.g., in a closed world scenario and with only 5 labeled samples, \ourWF has $80\%$ accuracy on \lowbw traces while Triplet Fingerprinting (TF), the state-of-the-art low-data WF technique, reaches only $64.4\%$ in exact same setting.  
\ourWF also outperforms existing techniques in open world scenario, e.g., when using 5 labeled samples, \ourWF reaches $92\%$ precision while Deep Fingerprinting has only $75\%$ precision. 
\end{comment}

% ------------------------------------------------------------------
\begin{comment}
We also evaluate \ourWF against Blind Adversarial Perturbations (BAP)~\cite{nasr2021defeating} countermeasure method which is based on adversarial examples and is shown to be effective defending WF attacks. Based on our results, \ourWF is more robust against existing systems when BAP is active, e.g., the accuracy of \ourWF reduces by $4.9\%$ when there are 10 labeled samples while the accuracy of DF decreases by $52.3\%$. 
\end{comment}
% ------------------------------------------------------------------

In summary, we made the following contributions in this work:
\begin{itemize}
    \item We propose a new direction in evaluating WF attacks in a realistic scenario where we perform all the training on traces collected in stable network conditions and then we evaluate the WF classifier on traces collected in poor network conditions or with time gaps.
    \item We designed and implemented \ourWF, a WF technique based on contrastive learning and data augmentation. \ourWF outperforms previous systems, particularly in a realistic scenario where the model is evaluated over traces with distributions unseen in the training phase. 
    \item We propose \aug, an augmentation algorithm that is tailored to the specific domain of Tor traces. \aug reflects different variations that may occur to Tor traces in realistic conditions such as concept drift and dynamic network conditions. 
    \item We perform extensive experiments to evaluate \ourWF in both closed world and open world scenarios. To assess the practicality of \ourWF, we train \ourWF using traces collected in consistent network conditions and then evaluate it on traces collected with a 6 years time gap and in both consistent and poor network conditions to simulate the effect of concept drift and dynamic network conditions.
    
\end{itemize}




==> misc/intro-01.tex <==
% ----------------------------------------------------------- Meeting:
% Main issue is collect on one setting and test on another one -> limited collection capability. 

% In any practical setting it is infeasible to collect traffic in any scenario. 

% Big solution is aug. the attacker has no option but to collect. We argue that to overcome, the approach is to do network augmentation

% Aug in other context
% We want to show that a tailored aug can help WF learn in unobserved setting. 
% Big contribution is to how to do augmentation

% Aug can be used in different network setting -> semi and self
% Instantiate aug through semi and self
% We want to reduce the less reliability on labeled data
% Summarize the big advantage. 
% Maybe say observed and unobserved for the results. 


%  ⁃ Aug: we start by naive approach then we show the tailored is better
%  ⁃ Argue the need to do aug in different traffic analysis settings


% Data collection and Experimental setting
% Bold texts for main results -> experiment section

% Maybe mentioning intrusion detection
% -------------------------------------------------------------

\section{Introduction}\label{sec:intro}
Anonymous communication systems hide the identities of the Internet end-points (e.g., websites) visited by Internet users, therefore protecting them against online tracking, surveillance, and censorship.
Tor~\cite{dingledine2004tor} is the most popular anonymous communication system in the wild with several million daily users~\cite{tor-metric}. 
Tor provides anonymity by relaying clients' traffic through cascades of proxies, known as relays.
% , known as circuits. 
A major threat to the anonymity provided by Tor and similar anonymity systems is a class of attacks known as \emph{Website Fingerprinting (WF)}~\cite{sirinam2018deep, sirinam2019triplet, cherubin2017website, cherubin2022online, oh2021gandalf, rimmer2017automated, panchenko2011website, cai2012touching, wang2013improved, panchenko2016website, hayes2016k, wang2016realistically, oh2019p1, var-cnn, 184463}. 
WF is performed by a passive adversary who monitors the victim's network traffic, e.g., a malicious ISP or surveillance agency. The adversary compares the victim's observed traffic trace against a set of pre-recorded website traces, to identify the webpage being browsed. 
% the adversary (e.g., a surveillance organization) trains a machine learning classifier on network traffic to target Internet websites, and uses such a classifier on the anonymized (e.g., Tor) traffic  of Internet users to infer the websites they are visiting. 
State-of-the-art (SOTA) WF attacks achieve significantly high accuracies  by leveraging deep neural network (DNN) architectures~\cite{oh2019p1, var-cnn, sirinam2018deep, sirinam2019triplet, cherubin2022online, rimmer2017automated, oh2021gandalf}, e.g., Deep Fingerprinting~\cite{sirinam2018deep} claims $98\%$ accuracy in a closed-world scenario.  

\paragraphb{Critiques of WF Studies:}
Despite the high accuracies claimed by SOTA WF attacks, several recent works~\cite{juarez2014critical, cherubin2022online, critique, wang2016realistically, wang2020high} have questioned the relevance of such attacks in practice due to the (unrealistic) threat models assumed in evaluating such attacks. Notably, the following are the major criticisms: 
\begin{itemize}
    \item \emph{Resilience to concept drift:} Concept drift refers to the phenomenon where the properties that distinguish one website from another can change over time. This can make it more difficult for WF techniques to accurately identify and track individual websites, as the features that were previously used to distinguish them may no longer be reliable. Juarez et al.~\cite{juarez2014critical} show that concept drift causes a significant drop in  WF accuracy.
    
    \item \emph{Network condition variations:} To collect ground truth data for training a WF classifier, researchers usually generate synthetic network traces through automated browsing of a pre-defined set of websites. However, during the deployment of the attack, the WF classifier may encounter traces that are collected in different network conditions (e.g., lower bandwidth). 
    % Various network conditions during training and deployment reduces the effectiveness of WF classifiers.
    
    \item \emph{Inaccurate user imitation:} Automated browser crawlers such as Selenium~\cite{selenium} are used by researchers to collect ground truth traces.
    The diversity of browser configurations and variations in user behavior such as visiting subpages of a website cannot be replicated by these crawlers.
    
    \item \emph{Requiring large labeled datasets:} Some DNN-based WF techniques require large amounts of labeled data for training to achieve high accuracies. 
\end{itemize}

In response to above criticisms, researchers proposed various heuristic techniques~\cite{cherubin2022online, wang2016realistically, oh2021gandalf, panchenko2016website, rimmer2017automated, wang2020high, pulls2020website} in the design and evaluation of WF attacks. For instance,  Wang and Goldberg~\cite{wang2016realistically} propose to maintain a fresh training set to make the model robust against concept drift. Furthermore, to improve WF accuracy when limited labeled data is available, \gandalf~\cite{oh2021gandalf} and Triplet Fingerprinting (TF)~\cite{sirinam2019triplet} use generative networks and metric learning, respectively. 
Most recently, Cherubin et al.~\cite{cherubin2022online} aim to address the issue of inaccurate user imitation by training a WF classifier on genuine Tor traces collected from exit Tor relays.  

\paragraphb{Enabling WF under realistic settings:}
We argue that the (ad hoc) approaches mentioned above either only partially address the issue, or are impractical themselves. For instance, the SOTA works of  \gandalf~\cite{oh2021gandalf} and Triplet Fingerprinting (TF)~\cite{sirinam2019triplet} only address the issue of data availability, but not concept drift. 
In this work, we aim to go after \textbf{the root cause} of the issues with WF techniques: \emph{lack of a longitudinal perspective into network traffic during training WF classifiers}. That is, the WF party is either not able to  collect enough (labeled) training  data to represent the diverse and volatile nature of the web traffic over time, or the collected training data only represents a specific threat model, e.g., a specific network condition, a particular Tor circuit, or a specific time frame. 
% However, the root cause of the problems mentioned above is the lack of access to traces in different settings. 
For instance, the adversary may collect Tor traces in one setting during training but may encounter traces in a completely different setting during the deployment that have not been previously observed. 
One potential solution to mitigate this issue is to collect Tor traces in a variety of network settings and scenarios. 
However, there can be an infinite number of settings and in any practical WF scenario, it is infeasible to collect traces in all possible settings, e.g., to solve the concept drift problem, the attacker needs to re-train the classifier regularly because the contents or even the layout of the websites may change everyday. 

In this work, we aim to address this root cause through \emph{augmentation of network traces}. Augmentation is to modify the existing samples to generate new samples that have the crucial features of the original ones. Our work is inspired by the successful  uses of  data augmentation in various SOTA machine learning architectures, in particular in various emerging semi-supervised and self-supervised applications. 
Our intuition is that augmenting network traces (e.g., of website connections) can help enhance the longitudinal perspective of a WF classifier, by enabling it to obtain network data samples that represent unobserved network conditions or settings. 
However, one can not simply borrow data augmentation techniques designed for classical machine learning tasks like vision. Instead, to get the most out of augmentation, we develop augmentation techniques that are tailored to the specific characteristics of network traffic. 

We demonstrate the impact of data augmentation on boosting the performance of WF attacks under realistic settings. 
We start by evaluating the impact of a naive augmentation approach, i.e., 
 randomly flipping the directions of Tor cells in a Tor trace. 
We then evaluate our network-tailored augmentation mechanism,  \aug, which is  tailored to specific configurations of Tor traffic. 
\aug replicates the modifications that may happen in unobserved WF settings by manipulating bursts of cells in a Tor trace. In our experiments, we show that \aug performs significantly better than a naive (random) augmentation.


\paragraphb{Deploying Network Augmentation:}
Augmented Tor traces can be used in different ways to train a WF classifier.
In this work, we instantiate \aug through semi-supervised learning (\semi) and self-supervised learning (\self). We use \semi and \self to reduce the dependency of the model on collecting large amounts of labeled data.  
After evaluating several deployments of \self and \semi techniques, we propose \ourWF, a WF attack based on \self techniques integrated with \aug. 
\ourWF learns useful representations of Tor traces without any requirement of labeled data as a pre-training phase.
We then fine-tune the pre-trained base model to adjust \ourWF to downstream datasets.
To evaluate \ourWF in a realistic scenario, we perform pre-training and fine-tuning using traces collected in one setting, and perform the attack on traces collected in different settings. 
We split our datasets into two categories:  traces collected in consistent network conditions (\textit{\highbw} traces), and  traces collected in poor and low bandwidth network conditions (\textit{\lowbw} traces). 


\paragraphb{Evaluations:}
We perform extensive experiments to evaluate \ourWF in both \textit{closed-world} and \textit{open-world} WF scenarios.
We show that \ourWF outperforms previous WF techniques when the traces for training and deployment are collected in different settings, e.g., in a closed-world scenario and with only 5 labeled samples, \ourWF has $80\%$ accuracy on \lowbw traces while Triplet Fingerprinting (TF), the SOTA low-data WF technique, reaches only $64.4\%$ in an exact same setup.
Furthermore, our results show that \ourWF shows more resilience to \drf compared to previous systems, e.g., when evaluating \ourWF on a dataset with a 5-year gap from the dataset used in pre-training, \ourWF reaches $72\%$ accuracy using 20 labeled samples while TF only reaches $51\%$ accuracy. 
\ourWF is also effective in an open-world scenario, e.g., when using 5 labeled samples, \ourWF reaches $92\%$ precision while Deep Fingerprinting has only $75\%$ precision.

We also evaluate \ourWF against the Blind Adversarial Perturbations (BAP)~\cite{nasr2021defeating} countermeasure technique which is based on adversarial examples and is shown to be effective in defending WF attacks. Based on our results, \ourWF is more robust compared to existing systems when BAP is active, e.g., the accuracy of \ourWF reduces by $4.9\%$ when there are 10 labeled samples while the accuracy of DF decreases by $52.3\%$. 

\paragraphb{Summary of contributions:} 
\begin{compactitem}
    \item This work is the first to investigate augmentation of network traffic to address realisticness issues of WF techniques; follow-up studies may extend this to other types of traffic analysis. 
    \item We deploy our network augmentation mechanisms into novel WF techniques that are based on semi-supervised and self-supervised mechanisms. 
    \item We perform extensive experiments in closed-world and open-world settings, demonstrating the superiority of our WF attacks in realistic settings. 
\end{compactitem}

==> misc/problem-00.tex <==

\section{Problem Statement}\label{problem}
\red{Maybe we can call this "threat model". Right now this is very similar to the introduction.}

% \red{Maybe we should combine this section with the background section}

% \red{Using genuine in some places instead of different network conditions}

WF attacks on Tor enable an adversary to predict which website a user is visiting by passively observing their encrypted traffic.  
The adversary chooses a subset of websites visited by users as the \emph{monitored} websites and is only interested in them. The rest of the websites visited by users are \emph{unmonitored} websites. 
In traditional WF attacks, the adversary first trains a machine learning classification model (mostly deep learning in recent works) and then deploys the model against users' traffic. Figure~\ref{fig:wf} shows the setting of a machine learning-based WF attack. 

\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{images/WF-training-test.pdf}
  \caption{Setup of a traditional WF attack based on machine learning.}
  \label{fig:wf}
\end{figure}

In traditional WF attack models, the adversary uses an entry-side vantage point for both the training and the attack phases as shown in Figure~\ref{fig:wf}. However, any researchers or adversary with this vantage point cannot collect ground truth website labels due to the protection provided by Tor's encryption and routing.
To obtain labeled Tor traffic, researchers use an automated Tor browser and crawl different websites to simulate a Tor client's browsing behavior and generate synthetic traffic traces for which they know the label.
As mentioned in~\cite{cherubin2022online}, synthetic traffic traces prevent researchers from understanding the capability of WF attacks against Tor. Traffic traces collected by automated browsers in isolated environments do not represent the diversity of actual Tor traces users generates. 
Previous works elaborated on the main reasons why the synthetic data is not diverse and thus we just mention them here briefly.
\begin{itemize}
    \item Using automated browser crawlers (researchers usually use Selenium~\cite{selenium}) with fixed browser configuration is not a proper example of actual Tor users. 
    
    \item Although the synthetic data generation happens in different batches, the network condition of the browsing usually remains consistent while Tor users in different locations experience different network conditions. 
    
    \item A common problem of synthetic traces, which is known as Concept Drift, is that the traces are collected from a \emph{static world} can quickly become outdated as the contents of the websites change rapidly. A trained model on a set of websites in a certain period of time does not take concept drift into account when evaluated on the same websites visited couple of weeks later. 
\end{itemize}


Another downside with recent WF attacks which is a problem for most learning-based techniques is the requirement of large amount of labeled data.
Recent studies~\cite{sirinam2019triplet, var-cnn, oh2021gandalf} address this problem using various limited-data machine learning techniques as mentioned in Section~\ref{back}.
The problem of synthetic trace generation and the requirement of large labeled data make the existing WF attacks not realistic in real-world scenarios.
Synthetic traces may not accurately represent the diverse network conditions that Tor circuits or users may encounter during actual deployment. Low-bandwidth traces and varying circuits are examples of conditions that may not be captured by conventional WF classifiers trained on synthetic website traces.
In Section~\ref{exp}, we show that using synthetic traces with stable and consistent network conditions in the training phase will results in a low performance of the classifier when tested with traces of poor network conditions which can happen usually for Tor users as they are mostly located in censored geographical locations with not-perfect network conditions. 

One possible way to overcome this problem is to use genuine Tor traces generated by actual users during the training phase. Cherubin et al.~\cite{cherubin2022online} replaced the traditional training phase of WF attacks by an online training phase that collects genuine Tor traces from an exit relays. They collect the genuine traces from Tor exit relays while preserving the safety and ethical regulations under the supervision of the Tor Project members. 
However, collecting traffic from an exit relay may not be feasible for the attacker since Tor usually assigns more trusted clients as exit relays. 
Furthermore, the attacker cannot access to ground truth data using only traces collected from an exit relay. 


In this work, we consider a realistic scenario for a WF attack and apply semi-supervised and self-supervised techniques to the specific constraints and configuration of the network traffic domain to address the limitations of traditional WF attacks. 
Based on the mentioned methods, we propose \ourWF, a WF technique that can achieve high accuracies in realistic and practical scenarios.
We posit that in a realistic scenario for WF attacks, adversaries train their classifier on synthetic traces collected under optimal network conditions with low latency and appropriate circuit bandwidths, which we refer to as \textit{\highbw traces}. 
During attack deployment, we encounter genuine Tor traces generated by users browsing websites under various network conditions. Some of these traces may be generated under conditions similar to those of the synthetic traces used by the adversary to train the WF classifier, while others may be generated under poor conditions, which we refer to as \lowbw traces.
For a realistic evaluation of our proposed attack, we use \highbw traces for our training part and use both \lowbw and \highbw traces for evaluation to show that 

Furthermore, for both semi-supervised and self-supervised techniques, data augmentation plays a critical role as it gathers more data points and also helps the model to learn the unseen distributions of Tor traces the attacker can face in the deployment phase. In Sections~\ref{semi} and \ref{self} we explain how these augmentation are important in both semi-supervised and self-supervised learning techniques. 
% In our work, as well as enabling the adversary to perform a WF attack with limited labeled data, data augmentation helps him to generate traces that can represent network traces with unseen network conditions. 
In Section~\ref{sec:aug}, we propose \aug, an augmentation algorithm that is tailored to the specifications of network traces domain. \aug can generate traces that are representative of genuine Tor traces that are not present in the synthetic dataset. 
We then show that using a sophisticated augmentation, the model gain the ability to identify traces with distributions that were not present in the training process.
% Note that even though augmentation still generates synthetic traces, using a well-designed augmentation can reflect the different conditions that may happen in the deployment phase. 

% ------------------------------------------------------------
\subsection{Concept Drift}
In a dynamic environment, the distribution of the target variable that a machine learning model learns can be non-stationary and therefore change over time, impacting the performance of the model when deployed. In the literature, this change in the distribution is referred to as dataset shift~\cite{morenotorres2012drift} or concept drift~\cite{gama2014conceptsurvey}.
% Using the terminology of Moreno-Torres et al.~\cite{morenotorres2012drift}
In the classification context, a problem can be defined by a set of covariates $X$, denoting the features, a class (target) variable $y$, and a joint distribution $P(y,X)$ referred to as concept, which can be written as $P(X|y)P(y)$. Therefore, concept drift between time $t_0$ and time $t_1$ can be defined as $\exists X: P_{t_0}(X,y) \neq P_{t_1}(X,y)$, where $P_{t_i}(X,y)$ denotes the joint distribution between X and y at time $t_i$ for $i \in \{0,1\}$. \textit{Real concept drift} is the changes in $P(X|y)$ between $t_0$ and $t_1$ which can happen whether $P(y)$ changes or not. \textit{Virtual concept drift}, also referred to as \textit{covariate shift} and \textit{feature change} happens if $P(X)$ changes between $t_0$ and $t_1$ but $P(y|X)$ does not change.


The data we use for our experiments consists AWF, a large dataset collected in 2017~\cite{rimmer2017automated}, as well a smaller Drift dataset that we collect 5 years later.
Over time, the content of a website change and can be completely different after 5 years, e.g. its back-end can be different resulting in a different loading time. Yet, it still has the same class label (URL), meaning $P(X|y)$ changes over time. Therefore, a deployed WF model needs to be resilient to real concept drift.
Note that this requirement exists whether or not the WF model uses offline learning or online learning. Traditional WF attacks ~\cite{oh2021gandalf, sirinam2019triplet, var-cnn, rimmer2017automated} use offline learning where all of the training data is available at the time of model training. Cherubin et al. ~\cite{cherubin2022online} propose using online learning, where the deployed model is continuously updated as more training data arrives. In either case, in a non-stationary and dynamic environment, the data evolves over time as the content of websites change and new websites are added to the monitored set. Therefore, $P(X|y)$ is changing over time.

Furthermore, our method of collecting traffic and extracting Tor cells for generating traces of a website slightly differs from that of \cite{rimmer2017automated}. For instance, the amount of time we wait for each website to load is different. Consequently, the distribution of traces collected for the same website can vary between the two datasets, even if everything else is the same. In this case, $P(X)$ has changed, but $P(y|X)$ has not changed. This is an instance of virtual concept drift to which our WF model should be resilient.

==> misc/semiself.tex <==
\section{Limited-Data Learning}\label{semiself}
In this section, we give a brief description of semi-supervised and self-supervised learning in computer vision and how they are the core of \ourWF.

\subsection{Semi-Supervised Learning}\label{semi}
Semi-supervised learning (SSL) is an approach to machine learning that combines a small amount of labeled data with a large amount of unlabeled data during training. SSL mitigates the requirement for labeled data by providing a means of leveraging unlabeled data. 
There is a line of research in semi-supervised learning aiming at producing an artificial label for unlabeled samples and training the model to predict the artificial label when fed unlabeled images as input~\cite{lee2013pseudo, mclachlan1975iterative, xie2020self, rosenberg2005semi, scudder1965probability}. These approaches are called pseudo-labeling. 
Similarly, consistency regularization~\cite{bachman2014learning, laine2016temporal, sajjadi2016regularization} obtains an artificial label using the model's predicted distribution after randomly modifying the input or model function. 
FixMatch~\cite{sohn2020fixmatch} is a recent semi-supervised algorithm in computer vision that combines consistency regularization and pseudo-labeling and performs a separate \textit{weak} and \textit{strong} augmentation when performing consistency regularization. 
FixMatch produces pseudo labels based on a weakly-augmented unlabeled sample which is used as a target when the model is fed a strongly-augmented version of the same input.
Note that in computer vision, augmentation refers to distorting the pixels of an image to generate new samples with the same label. This includes making small changes to images or using deep learning models to generate new data points. 
In FixMatch, weak augmentation is a standard flip-and-shift augmentation strategy while strong augmentation is based on an algorithm called AutoAugment~\cite{cubuk2019autoaugment}.
However for network traces, due to their underlying protocol constraints and the nature of the packets augmentation is challenging. We will discuss our augmentation strategy in Section~\ref{sec:aug}.  
Figure~\ref{fig:fixmatch} shows how FixMatch works when fed with network traces.

\begin{figure*}[t]
  \centering
  \includegraphics[width = 0.8\linewidth]{images/fixmatch.pdf}
  \caption{Diagram of FixMatch when fed with network traces}
  \label{fig:fixmatch}
\end{figure*}


For an $L$-class classification problem, let $\mathcal{X} = \big\{ (x_b,p_b): b \in (1,\cdots,B) \big\}$ be a batch of $B$ labeled samples, where $x_b$ are the training network traces and $p_b$ are one-hot labels. 
Let $\mathcal{U} = \big\{  u_b: b \in (1, \cdots, \mu B) \big\}$ be a batch of $\mu B$ unlabeled traces where $\mu$ is a hyperparameter that denotes the ratio of number of unlabeled samples ($\mathcal{U}$) to labeled samples ($\mathcal{X}$). 
We assume $p_m (y|x)$ is the predicted class distribution produced by the traffic analysis model for input $x$ and $H(p,q)$ denotes the cross-entropy between two probability distributions $p$ and $q$. 
Similar to FixMatch, we perform two types of augmentations: strong and weak, denoted by $\mathcal{A}(.)$ and $\alpha(.)$ respectively. 
Our loss function consists of two cross-entropy loss terms: a supervised loss $\ell_s$ applied to labeled data and an unsupervised loss $\ell_u$. 
In particular, $\ell_s$ is the standard cross-entropy loss used in traffic analysis classification scenarios (i.e., Website Fingerprinting) on weakly augmented labeled samples:

\begin{align}
    \ell_s = \frac{1}{B} \sum_{b=1}^{B} \text{H} \big( p_b,p_m(y | \alpha(x_b)) \big)
\end{align}

As mentioned earlier, for each unlabeled sample, FixMatch generates a pseudo label which is then used in a standard cross-entropy loss. Given a weakly-augmented version of an unlabeled sample $q_b = p_m (y | \alpha(u_b))$, we compute the model's predicted class distribution. We then use $\hat{q}_b = \arg\max(q_b)$ as a pseudo-label, except we apply the cross-entropy loss against the model's output for strongly-augmented version of $u_b$:

\begin{align}
    \ell_u = \frac{1}{\mu B} \sum_{b=1}^{\mu B} \mathbb{1}\big(\max(q_b) \geq \tau_f \big) \text{H}\big( \hat{q}_b, p_m (y | \mathcal{A}(u_b)) \big)  
\end{align}

\noindent where $\tau_{f}$ is a scalar hyperparameter indicating the threshold above which we retain a pseudo-label. We minimize the following loss: $\ell_s + \lambda_u \ell_u$ where $\lambda_u$ is a fixed scalar hyperparameter denoting the relative weight of the unlabeled loss. 


\subsection{Self-Supervised Learning}\label{self}
Self-supervised (Unsupervised) representation learning tries to learn useful embeddings from unlabeled data. 
Contrastive Learning is a subset of unsupervised learning that aims to learn embeddings by enforcing similar elements to be equal and dissimilar elements to be different. 
SimCLR~\cite{chen2020simple} is a recent framework in computer vision for contrastive learning of visual representations. In particular, SimCLR learns representations (embeddings) of unlabeled data by maximizing agreement between differently augmented views of the same data example via a contrastive loss in the latent space. 
Similar to semi-supervised learning, we will discuss augmentation in network traffic domain in Section~\ref{sec:aug}. 
We apply SimCLR to traffic analysis algorithms to learn embeddings of network traces where there is no labeled data is available. 
Figure~\ref{fig:simclr} shows the general framework of SimCLR adjusted to traffic analysis domain. SimCLR framework comprises the following four major components:
\begin{itemize}
    \item A stochastic data augmentation module that transforms any given network trace $x$ resulting in two correlated views of the same trace, denoted $\tilde{x}_i$ and $\tilde{x}_j$, which we consider as a positive pair. 
    \item A neural network base encoder $f(.)$ that extracts embeddings from augmented network traces. We use the underlying neural works used in traffic analysis algorithms to obtain $e_i = f(\tilde{x}_i)$ where $e_i \in \mathbb{R}^d$ is the output of the underlying neural network before the last layer (The fully connected layer that generates the output probabilities); $e_i$ also represents the network trace embedding extracted by the base model. 
    \item A small neural network \textit{projection head} that maps embeddings to the space where contrastive loss is applied. Similar to SimCLR, we use a fully connected network with one hidden layer to obtain $z_i = g(e_i) = W^{(2)}\sigma (W^{(1)}e_i)$ where $\sigma$ is a ReLU non-linearity. 
    \item A \textit{contrastive loss} function to maximize the agreement between augmented versions of an unlabeled sample. Given a set $\{ \tilde{x}_k \}$ including a positive pair of examples $\tilde{x}_i$ and $\tilde{x}_j$, the contrastive prediction task aims to identify $\tilde{x}_j$ in $\{ \tilde{x}_k \}_{k \neq i}$ for a given $\tilde{x}_i$.  
\end{itemize}


\begin{figure*}[t]
  \centering
  \includegraphics[width = 0.8\linewidth]{images/simclr.pdf}
  \caption{Diagram of SimCLR when fed with network traces}
  \label{fig:simclr}
\end{figure*}

SimCLR randomly samples a minibatch of $N$ network traces and apply contrastive loss on pairs of augmented samples generated from the minibatch, resulting in 2$N$ network traces. To construct the negative traces, given a positive pair, SimCLR considers the other 2$(N-1)$ augmented traces within a minibatch as negative samples. If we assume $\text{sim}(u, v) = u^T v / \lVert u \rVert \lVert v \rVert$ denotes the dot product between $\ell_2$ normalized of vectors $u$ and $v$ (i.e. cosine similarity), the contrastive loss function for a positive pair of traces $(i, j)$ is defined as:

\begin{align}\label{eq:contrasive-loss}
    \ell_{i,j} = - \log \frac{\exp(\text{sim}(z_i, z_j)/\tau_s)}{\sum_{k=1}^{2N} \mathbb{1}_{[k\neq i]}\exp (\text{sim}(z_i, z_k)/\tau_s)}
\end{align}

\noindent where $\mathbb{1}_{[k\neq i]} \in \{0,1\}$ is an indicator function evaluating to 1 iff $k \neq i$ and $\tau_s$ denotes a temperature parameter. The SimCLR work term this loss \textit{NT-Xent} (the normalized temperature-scaled entropy loss).

